Evaluation of OpenAI Codex for HPC Parallel Programming Models Kernel Generation

We evaluate AI-assisted generative capabilities on fundamental numerical kernels in high-performance computing (HPC), including AXPY, GEMV, GEMM, SpMV, Jacobi Stencil, and CG. We test the generated kernel codes for a variety of language-supported programming models, including (1) C++ (e.g., OpenMP [including offload], OpenACC, Kokkos, SyCL, CUDA, and HIP), (2) Fortran (e.g., OpenMP [including offload] and OpenACC), (3) Python (e.g., numba, Numba, cuPy, and pyCUDA), and (4) Julia (e.g., Threads, CUDA.jl, AMDGPU.jl, and KernelAbstractions.jl). We use the GitHub Copilot capabilities powered by OpenAI Codex available in Visual Studio Code as of April 2023 to generate a vast amount of implementations given simple <kernel> + <programming model> + <optional hints> prompt variants. To quantify and compare the results, we propose a proficiency metric around the initial 10 suggestions given for each prompt. Results suggest that the OpenAI Codex outputs for C++ correlate with the adoption and maturity of programming models. For example, OpenMP and CUDA score really high, whereas HIP is still lacking. We found that prompts from either a targeted language such as Fortran or the more general-purpose Python can benefit from adding code keywords, while Julia prompts perform acceptably well for its mature programming models (e.g., Threads and CUDA.jl). We expect for these benchmarks to provide a point of reference for each programming model's community. Overall, understanding the convergence of large language models, AI, and HPC is crucial due to its rapidly evolving nature and how it is redefining human-computer interactions.

==> X5.laris.tex <==

\begin{figure}[t]%[bp]
\begin{center}
%\includegraphics[width=1\linewidth]{figures/diagram/iris-blas.png}
\includegraphics[width=1\linewidth]{figures/diagram/laris-iris-blas.png}

%\includegraphics[width=1\linewidth]{figures/diagram/laris.png}

%\includegraphics[width=1\linewidth]{figures/diagram/lufactorization.pdf}
\end{center}
  \vspace{-0.1in}
\caption{Software stack and design of LaRIS.}
%\caption{IRIS-BLAS: a portable BLAS library on IRIS run time}
\label{fig:laris}
  \vspace{-0.2in}
\end{figure}

\section{LaRIS: Design and Objectives}
\label{label:laris}
LaRIS (an LAPACK library on the IRIS run time) is designed with three goals in mind: (1) simplify performance portability of LAPACK code on heterogeneous systems, (2) exploit the computational capabilities of heterogeneous systems to the fullest by using automatic tiled algorithms, and (3) facilitate the inclusion of algorithm-specific performance models to guide scheduling in heterogeneous systems. The LaRIS software stack is shown in Fig.~\ref{fig:laris}.
%We implemented LaRIS (a LAPACK library on IRIS run time) to simplify the performance portability of LAPACK code on extremely heterogeneous systems. 

\subsection{Enabling Portability}
To make LaRIS portable, we separated the algorithm design from the tuning. Algorithm design involves expressing the tiled LAPACK algorithms by using tasks and their dependencies, and tuning consists of choosing the target kernels and processors for executing each of the tasks. Two levels of abstractions facilitated by the IRIS run time and the IRIS-BLAS library enable such a separation (Fig.~\ref{fig:laris}). Tiled LAPACK algorithms are expressed by using type-less LaRIS APIs along with the IRIS run time and the IRIS-BLAS APIs that do not include any architecture- or vendor-library specific detail (see Listings~\ref{lst:getrf_code} and ~\ref{lst:gemm_code} in \nameref{sec:appendix1}). Therefore, LaRIS codes are completely agnostic of the architecture and vendor library at compile time. This feature facilitates the implementation of different tiled algorithms for LAPACK codes without having to worry about vendor libraries or the underlying hardware.

Tuning occurs at run time. By using dynamically linked libraries of IRIS and IRIS-BLAS at run time, LaRIS tasks are scheduled on different processors in a heterogeneous system on which vendor-specific kernels suitable for those processors are executed. IRIS's run time scheduler enables the full orchestrations during which IRIS-BLAS dynamically provides the vendor-specific tuned kernels. Thus, the tuning phase does not require code modifications at the algorithm level, but they are conducted internally and transparently by IRIS for each task. Leveraging IRIS's dynamic scheduler, the set of tasks in a LaRIS algorithm attempts to obtain the maximum performance on the target architecture by maximizing the use of all the computational resources available in a heterogeneous system.


\subsection{Tiled Execution}
When processing larger matrix sizes, tiling is required to utilize all the processors in a heterogeneous system. LaRIS provides APIs for automatic tiling and reconstructing. Tiling occurs before task and dependency creation. While creating the graph, LaRIS associates memory chunks for different tiles to different tasks. 

\subsection{Current Status}
LaRIS is under development along with IRIS-BLAS to support more LAPACK and BLAS-level functionalities. Although performance model--guided scheduling is in progress, the current implementation has enough support to make LAPACK codes portable for tiled execution. The following sections demonstrate one such capability with tiled LU factorization as a test case.

==> X6.lu_methodologies.tex <==
\begin{figure*}[!th]
 \centering
  \vspace*{-1em}
  %\includegraphics[width=1\textwidth,scale=1.0,keepaspectratio]{figures/8x8_colors_corrected.eps}
  
  %\includegraphics[width=1\textwidth,height=10cm]{figures/8x8_processed.eps}
  \includegraphics[width=1\textwidth,height=12cm]{figures/diagram/8x8_colors_corrected.eps}
  \vspace{-.25in}
  \caption{DAG of an $8\times8$ LU factorization that creates $204$ tasks and their dependencies. Red ellipses are GETRF, orange ellipses are TRSM, and blue ellipses are GEMM.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
  \vspace{-.2in}
 \label{fig:dag}
\end{figure*}



%\section{Methodologies}
\section{Tiled LU Implementation in LaRIS}
\label{label:methodologies}


%\subsection{Tiled LU implementation in LaRIS}

%LARIS and it's objective : Pedro \\
%			§ LU factorization as a proof of concept
%\subsection{Task based LU factorization challenges}
%\subsection{LU factorization Algorithm}
%    		§ Task figures : Pedro \\
%			§ LU factorization algorithm: Monil or Pedro \\
%			§ Accuracy check algorithm: Monil
%\subsection{Math library function discussion and reasoning:}
%            Math library function discussion and reasoning: Pedro and Monil \\
%			§ Why column major
%\subsection{A Flow description of LU factorization with DAG from IRIS:}: Monil

%Listing~\ref{lst:dgetrf_code} shows the pseudocode for the IRIS-implemented LU factorization. 
This section discusses the LU factorization algorithm implemented in LaRIS. LaRIS decomposes a matrix into a set of square tiles (Fig.~\ref{fig:npgetrf_schema}). Based on the provided tile configuration at the LaRIS level, the algorithm decomposes the problem by using different memory spaces, tasks, and dependencies. The pseudocode of the type-less LU factorization implementation in LaRIS can be found in Listing~\ref{lst:getrf_code} in \nameref{sec:appendix1}.

\subsection{Tasks}
The implementation of LU factorization in LaRIS consists of four different tasks: 
\begin{enumerate}[label={(\arabic*)}]
    \item GETRF, in which LaRIS computes a no-pivoting LU factorization on the diagonal tile of the matrix. 
    \item TRSM-top, in which LaRIS computes the level-3 BLAS TRSM routine by using the lower side of the LU factorization computed in the previous task as the input matrix and a set of tiles located at the right of the LU matrix as the output matrices. One task per tile is created for computation. 
    \item TRSM-left, in which LaRIS computes the same level-3 BLAS operation used in the previous tasks; however, it computes a different part of the matrix where the input is the upper side of the LU matrix processed by the first task (GETRF) and outputs a set of square tiles located under the lower side of the LU matrix. 
    \item GEMM, in which LaRIS computes a set of matrix-matrix multiplications by using the output of the two previous tasks (TRSM-top and TRSM-left) as input and the tiles that correspond to the remaining matrix parts as output. LaRIS computes all the previous tasks until the entire matrix is computed (Fig.~\ref{fig:npgetrf_schema}).
\end{enumerate}






\subsection{Automated DAG Creation and Scheduling}
After tiling the memory, LaRIS creates a DAG that contains the number of tasks and the dependencies between these tasks. Because the execution environment is dynamic, incorrect dependencies lead to inaccurate results. In LU factorization, parallelization is possible between the tasks from different iterations. Therefore, LaRIS follows data dependency instead of task dependency, where a dependency between two tasks is created if and only if the output memory of one task is an input memory of another. 

Once the graph is created, LaRIS starts the execution by using \texttt{iris\_graph\_submit}. For the sake of completeness, Fig.~\ref{fig:dag} shows the DAG created by LaRIS LU code for a tile configuration (i.e., matrix decomposition) of $8\times8$ for a matrix of size $16,384\times16,384$. LaRIS is currently capable of computing the correct result of the LU factorization by decomposing a matrix with a tile configuration of up to $64\times64$, which creates $89,440$ kernel tasks. After the graph is submitted, the IRIS run time reads the task graph and submits them to the task queue. IRIS's dynamic task scheduling policy takes the tasks from the queue, chooses a target processor based on the policy, and submits the task to the device-specific task pool for execution. 



%In LU factorization, parallelization is possible between the task of the same tile from different iterations


\subsection{Ensuring Utilization and Portability}

As described in Section~\ref{label:laris}, one of LaRIS's main goals is to maximize the utilization of all available computational resources. To do that, apart from carrying out the matrix decomposition illustrated in Fig.~\ref{fig:npgetrf_schema}, we use tuned multithreaded kernels (on CPU and GPUs) to exploit the parallelism at both algorithm and task levels. LaRIS leverages the dynamic scheduling policy from the IRIS run time to use all the available computational resources in a heterogeneous system. For example, the \texttt{iris\_any} dynamic scheduler assigns each task to a CPU or GPU device depending on its availability at run time. Hence, the task execution is completely decoupled from the programming, and its IRIS run time's job is to care for it. The application's performance depends on the number of tasks (i.e., tiles), computational cost of each operation (GETRF/TRSM, GEMM), the type of underlying computing resources, and their count.


Portability is ensured by associating each task in the graph with one generic LAPACK or BLAS API from IRIS-BLAS. The parameters of these routines are similar to the specification of standard math libraries (i.e., LAPACK, BLAS). Hence, dynamic loading of the appropriate vendor-library kernel becomes possible. For example, LaRIS's double-precision GETRF routine is dynamically linked to the \texttt{LAPACKE\_mkl\_dgetrfnpi} kernel of the MKL library if a CPU is chosen by the IRIS dynamic scheduler to execute the task. If the IRIS scheduler chooses an AMD GPU, then \texttt{hipblasDgetrf} from hipBLAS is executed. Therefore, tasks of the DAG shown in Fig.~\ref{fig:dag} can execute on any available processor by launching the tuned kernel for that architecture. Relying on this dynamic selection capability, the same LaRIS code can be ported to a different set of computing resources without even changing a line in the code.



\begin{table*}[!t]
%\vspace{-0.1 in}
\caption{Heterogeneous systems used in this research}
\vspace{-0.1 in}
%\small
\centering
%\setlength{\tabcolsep}{0.4em}
\begin{center}
%\begin{tabular}{| P{1.2cm} | p{6.8cm} |}

\begin{tabular}{|c|c|c|c|}
\hline
%\textbf{} &\multicolumn{3}{|c|}{\textbf{Heterogeneous systems}}  \\
%\hline
%\cline{2-5} 
 \textbf{Nodes} & \textbf{NVIDIA DGX-1} & \textbf{Frontier-like node} & \textbf{CADES node}\\
\hline
\textbf{Facility} & ExCL at ORNL & Crusher (early access) at ORNL & CADES at ORNL \\ \hline 
\textbf{} & Total 4 GPUs & Total 8 GPUs & Total 8 GPUs \\ 
\textbf{GPUs} & 4$\times$ NVIDIA V100 & 4$\times$ AMD MI250X & 4$\times$ NVIDIA A100 \\
\textbf{} &  & (each contains two) & 4$\times$ AMD MI100 \\ \hline 
\textbf{CPU} & Intel Xeon E5-2698, 20 cores & AMD EPYC 7A53, 64 cores  & AMD EPYC 7763, 128 cores\\ \hline 
\textbf{Compiler} & GNU-9.4.0 & GNU-8.5.0 & GNU-8.5.0\\ \hline 
\textbf{CUDA and ROCm versions} & CUDA-11.7 & CUDA-11.7 and ROCm-5.1.0 & CUDA-11.7 and ROCm-5.1.2\\ \hline 
\textbf{Math libraries for GPUs} & cuBLAS and cuSOLVER & hipBLAS  & cuBLAS, cuSOLVER and hipBLAS\\ \hline 
\textbf{Math libraries } & OpenBLAS-0.3.20 and & OpenBLAS-0.3.17 and  & OpenBLAS-0.3.20 and \\ 
\textbf{for CPU} & MKL-2022.1.0 & MKL-2020.4.304  & MKL-2020.4.304\\
\hline 

%Release year & 2016 & 2017 &  2020 & 2022   \\ \hline
%Architecture & Pascal & Volta &  Ampere & Hopper \\ \hline
%Number of SMs/CUs & 56 & 80 & 108  & 114   \\  \hline
%Number of cores & 3,584 & 5,120  & 6,912 & 14592\\  \hline
\end{tabular}

\label{table:systems}
\end{center}
\vspace{-0.2in}
\end{table*}

%\begin{figure*}[!th]
% \centering
  %\vspace*{-2.em}
  %\includegraphics[width=1\textwidth,scale=1.0,keepaspectratio]{figures/8x8_colors_corrected.eps}
  
%  \includegraphics[width=1\textwidth,height=10cm]{figures/8x8_processed.eps}
  %\includegraphics[width=1\textwidth,height=10cm]{figures/8x8_colors_corrected.eps}
%  \vspace{-.2in}
%  \caption{Same DAG. RED=GETRF, Orange=TRSM and Blue=GEMM
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
%   }
% \label{fig:dag}
%\end{figure*}

%\begin{figure}[!th]
% \centering
  %\vspace*{-2.em}
  %\includegraphics[width=1\textwidth,scale=1.0,keepaspectratio]{figures/8x8_colors_corrected.eps}
  
%  \includegraphics[width=.25\textwidth,height=5cm]{figures/3x3_processed.eps}
  %\includegraphics[width=1\textwidth,height=10cm]{figures/8x8_colors_corrected.eps}
%  \vspace{-.1in}
%  \caption{3x3 for demonstrating dependencies. RED=GETRF, Orange=TRSM and Blue=GEMM
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
%   }
% \label{fig:dag}
%\end{figure}


%\subsection{How it Works at Run Time}

%- Iris blas and iris dynamic linking
%- export IRIS\_ARCHS= to choose target device
%-- automatic parallelization


==> X7.experiment_setup.tex <==



\section{Experimental Setup}
\label{expr:setup}
For this work, we used three heterogeneous systems with CPUs and GPUs from different manufacturers located in different computing facilities at ORNL. Table~\ref{table:systems} shows the hardware configurations, architectures, compilers, software stacks, and BLAS libraries that were used. For profiling and tracing, the native capabilities of the IRIS run time were used. Execution times reported in Section~\ref{label:expr} are for the graph execution without the time spent for the initial memory allocation on the host side for matrix creation.

%Experimentation was done with matrix size of [$8192\times8192$, $16384\times16384$, $32768\times32768$, $65536\times65536$, $131072\times131072$] and tile sizes of [$8\times8$, $16\times16$, $32\times32$, $64\times64$]. The number of kernel task launched these tile configurations are [204, 1496, 11440, 89440].   

Experiments were conducted with tile configurations of [$4\times4$, $8\times8$, $16\times16$, $32\times32$, and $64\times64$], which resulted in [$30$, $204$, $1,496$, $11,440$, and $89,440$] tasks (kernels) to compute the final result. Double precision was used for all experiments. Experiments were run five times, and an average was reported.

==> X8.experiment.tex <==

\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}

  \subfloat[Trace from NVIDIA DGX-1.\label{subfig-1:dgx}]{
  %\includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/experiments/Equinox-32k-32_trace.png}
  \includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/experiments/equinox-16k-32.png}
  }
 \vspace{-.1in} 
   \subfloat[Trace from Crusher node.\label{subfig-1:crusher}]{
 \includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/experiments/crusher-16k-32_trace.png}
  }
     \vspace{-.1in}

   \subfloat[Trace from CADES node.\label{subfig-1:cades}]{
  \includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/experiments/mi100-16k-32_trace.png}
  }
   \vspace{-.05in}
   \caption{Evaluating portability and exploiting parallelism in GPUs and CPUs from multiple vendors. Traces are generated for a  $16,384\times16,384$ matrix with a tile decomposition of $32\times32$, which created $11,440$ tasks. Red is GETRF, orange is TRSM, and blue is GEMM. The horizontal axis shows the timeline only for graph execution in seconds, whereas the vertical axis shows different CPUs and GPUs. 
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool, and X axis = the stride size.
   }
 \label{fig:trace}
 \vspace{-1.5em}
\end{figure*}


\section{Experiments}
\label{label:expr}
We evaluated the efficacy of LaRIS's LU factorization in four steps. First, LaRIS's portability is explored. Then, strong scaling performance for an increasing number of GPUs is evaluated, followed by a discussion of the trade-off between parallelism and overhead. Finally, the optimization opportunities are identified. 


\subsection{Portability to Different Heterogeneous Devices}
\label{label:expr:port}
Two aspects are evaluated in this experiment: portability and system utilization. For this experiment, we used a $16,384\times16,384$ matrix with a tile decomposition of $32\times32$, which created $11,440$ kernel tasks.
Because one of the main objectives of LaRIS is to provide a portable solution for LAPACK codes, no architecture- or vendor-specific library changes were made in the LU factorization code while deploying and experimenting on the three heterogeneous systems mentioned in Table~\ref{table:systems}. Once the graph was submitted to the IRIS run time, seamless execution was observed in these systems (Fig.~\ref{fig:trace}). The IRIS run time was able to select appropriate vendor-specific BLAS kernels to schedule on the corresponding processors and orchestrate the correct result for the LU factorization. Because the \texttt{IRIS\_any} scheduling policy was used, no binding was imposed between the kernel types, BLAS kernel, or target processors. Therefore, IRIS had complete freedom to run any kernel on any device to maximize the parallelization opportunities.

Traces for these executions are shown in Fig.~\ref{fig:trace}. Figures~\ref{subfig-1:dgx} and~\ref{subfig-1:crusher} show the execution timeline on one CPU and on multiple GPUs from NVIDIA and AMD, respectively. Notably, the CPU bar represents all available cores. Figure~\ref{subfig-1:cades} shows the most interesting case in which one AMD CPU, four NVIDIA A100 GPUs, and four AMD MI100 GPUs processed the entire graph. The complete separation of the LAPACK code from the BLAS libraries and the architecture made this seamless portability possible.

Three traces in Fig.~\ref{fig:trace} also demonstrate system utilization by depicting $11,440$ task kernels in different colors. Conceptually, these traces can be considered a counter-clockwise, 90$^{\circ}$ rotation of Fig.~\ref{fig:dag} when using multiple processors. White spaces indicate idle time and are barely noticeable in all these three traces, except at the end of the timeline. As shown in Fig.~\ref{fig:dag}, parallelization reduces at the end of the LU factorization algorithm, which is why there are some white spaces at the very end. However, the main takeaway in terms of utilization is that when the algorithm exposed parallelism, LaRIS was able to utilize the parallelism by exploiting the computational power of all the available resources.

\subsection{Strong Scaling in a MultiGPU Environment} 
Strong scaling capability is evaluated in this experiment. The matrix size and tile configuration were kept the same as the number of GPUs used in the systems (Table~\ref{table:systems}) was increased. A $16\times16$ tile configuration was used for all the experiments. A matrix size of $16,384\times16,384$ was used for the DGX-1 machine, and $32,768\times32,768$ was used for Crusher and the CADES node. The number of GPUs was increased to observe the change in execution time, which is presented in Fig.~\ref{fig:expr:strong-scaling}. The DGX-1 machine showed a performance improvement with each addition of an NVIDIA V100 GPU for processing LU factorization (Fig.~\ref{subfig-2:dgx}). 

Scalability for the Crusher node is shown in Fig.~\ref{subfig-2:crusher}, and performance improvements were observed when adding up to four AMD MI250X GPUs. However, increasing the number of GPUs beyond four made the performance worse. %, indicating that the required data transfer overhead outweighed the benefit of parallelism. 

Scalability on the CADES machine showed a waterfall trend (Fig.~\ref{subfig-2:cades}). When the number of NVIDIA A100 GPUs was increased, the performance improvement was saturated when using four GPUs. However, the performance improvement kept resurfacing when AMD MI100 GPUs were added and reached a saturation point when four NVIDIA and four AMD GPUs were used. 

The saturation shown in Figs.~\ref{subfig-2:crusher} and \ref{subfig-2:cades} can be correlated to the overhead of multidevice tasking, which induces an increased number of memory transfers. With an increasing number of GPUs, the probability that the data needed by the tasks is not located in the device increases; hence, it can cause extra memory transfers. We are working toward better and more efficient memory management for such scenarios. 

%While the scalability experiments showed performance improvement, they also revealed the increasing amount of overhead originating from extra data transfers when the number of GPUs was increased.





\subsection{Best Tile Configuration: a Trade-off between Parallelism and Overhead} 
\label{label:expr:best-tile}
This experiment delves into finding the best tile configurations for a given matrix size in a node. Large matrices were processed by using different tile configuration launch-task kernels that ranged in number from $30$ (for $4\times4$) to $89,440$ (for $64\times64$) kernel tasks (Fig.~\ref{fig:expr:best-tile}). For this experiment, all the processing units were used. Some matrix and tile configurations are not shown because the available memory in the existing devices did not allow all configurations. 



\begin{table}[!t]
%\vspace{-0.1 in}
\caption{Best tile configuration for different matrix sizes}
\vspace{-0.1 in}
%\small
\centering
%\setlength{\tabcolsep}{0.4em}
\begin{center}
%\begin{tabular}{| P{1.2cm} | p{6.8cm} |}

\begin{tabular}{|c|c|c|c|}
\hline
%\textbf{} &\multicolumn{3}{|c|}{\textbf{Heterogeneous systems}}  \\
%\hline
%\cline{2-5} 
 \textbf{Matrix} & \textbf{DGX-1} & \textbf{Crusher node} & \textbf{CADES node}\\
\hline
%\textbf{Facility} & ExCL at ORNL & OLCF's Crusher at ORNL & CADES at ORNL \\ \hline 
\textbf{$8,192\times8,192$} & $8\times8$ & $4\times4$& $4\times4$ \\ \hline 
\textbf{$16,384\times16,384$} & $8\times8$ & $8\times8$ & $8\times8$ \\ \hline 
\textbf{$32,768\times32,768$} &  $8\times8$ & $16\times16$ & $16\times16$ \\ \hline 
\textbf{$65,536\times65,536$} & NA & $16\times16$  & $16\times16$\\ \hline 

%\hline 

%Release year & 2016 & 2017 &  2020 & 2022   \\ \hline
%Architecture & Pascal & Volta &  Ampere & Hopper \\ \hline
%Number of SMs/CUs & 56 & 80 & 108  & 114   \\  \hline
%Number of cores & 3,584 & 5,120  & 6,912 & 14592\\  \hline
\end{tabular}

\label{table:expr:best-tile}
\end{center}
\vspace{-0.2in}
\end{table}


\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}

   \subfloat[NVIDIA DGX-1 with four V100 GPUs.\label{subfig-2:cades}]{
  \includegraphics[width=.32\textwidth,scale=1.0,keepaspectratio]{figures/experiments/equinox-scal.png}
  }
  \subfloat[Crusher node with eight MI250X GPUs.\label{subfig-2:dgx}]{
  \includegraphics[width=.32\textwidth, scale=1.0,keepaspectratio]{figures/experiments/crusher-scal.png}
  }
   \subfloat[CADES node with four NVIDIA A100 GPUs and four AMD MI100 GPUs.\label{subfig-2:crusher}]{
  \includegraphics[width=.32\textwidth,scale=1.0,keepaspectratio]{figures/experiments/mi100-scal.png}
  }
  
   \vspace{-.05in}
   \caption{Strong scaling on different machines.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \vspace{-.1in}
 \label{fig:expr:strong-scaling}
 \vspace{-1em}
\end{figure*}

\begin{figure*}[!b]
 \centering
  \vspace{-2.em}

   \subfloat[NVIDIA DGX-1. \label{subfig-3:dgx}]{
  \includegraphics[width=.3\textwidth,scale=1.0,keepaspectratio]{figures/experiments/task_scalability_equinox.png}
  }
  \subfloat[Crusher node.\label{subfig-3:crusher}]{
  \includegraphics[width=.3\textwidth,scale=1.0,keepaspectratio]{figures/experiments/task_scalability_crusher.png}
  }
   \subfloat[CADES node.\label{subfig-3:cades}]{
  \includegraphics[width=.3\textwidth,scale=1.0,keepaspectratio]{figures/experiments/task_scalability_cades.png}
  }
  
   \vspace{-.05in}
   \caption{ Finding the best tile configuration for different matrix sizes when all the processing elements are used.
   %Trade-off between task parallelism vs. overhead dictates the best tile configuration for different matrix sizes when all the processing elements are used.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr:best-tile}
 %\vspace{-1.6em}
\end{figure*}


The main observation from Fig.~\ref{fig:expr:best-tile} is that the best tile configuration for different matrices varies from node to node because of the underlying hardware capacity. Table~\ref{table:expr:best-tile} presents a summary of findings shown in Fig.~\ref{fig:expr:best-tile} by showing the best tile configurations for different matrix sizes on different nodes. Only the $16,384 \times 16,384$ matrix has the same best tile configuration on all nodes. Moreover, the larger matrices prefer larger tiles on machines with more processing units. Such a preference is the byproduct of a node having more processing elements that can leverage the extra parallelism generated by the large tile configurations. However, no matrix performed the best for the configurations $32 \times 32$ and $64 \times 64$. We correlate such outcomes with the inclusion of host-to-device and device-to-host memory transfer for each task. Thus, a larger number of tasks in a larger number of processors incur more memory transfer overhead. Adding memory transfers is not required for every task because the parent task might have already brought the data to the device. We plan to optimize such data transfers in the future. 


\subsection{Opportunities} 
We have identified two opportunities from these experiments. First, we see that the best execution time does not depend on using the maximum number of available processors or the highest number of tiles. Every matrix configuration and node has a sweet spot for a particular tile and number of processors. Generating performance models to guide the scheduler to that desired tile and processor combination is a research opportunity. The second opportunity arises from the memory transfer inefficiency discussed in Section~\ref{label:expr:best-tile}.  






==> X9.conclusion.tex <==
\section{Conclusions and Future Work}
\label{label:conclusions}
In this paper, we presented LaRIS, a portable solution that enables LAPACK codes on all processing elements in a heterogeneous system by using tiled LAPACK algorithms. Using the IRIS run time and the IRIS-BLAS library, LaRIS decouples LAPACK algorithms from the architectures and architecture-specific tuned BLAS libraries. Moreover, LaRIS offers automatic tilling and can dynamically link to the corresponding vendor-provided BLAS kernel at run time, which enables LaRIS to be portable and capable of using all the processors in different heterogeneous systems. By launching $\approx90,000$ BLAS kernels for LU factorization, LaRIS demonstrated its ability to be portable to different heterogeneous systems, including a representative node of the first exascale supercomputer, ORNL's Frontier, and showed its capability to utilize all the processors simultaneously to compute correct results. Some optimization opportunities (e.g., memory optimization) were also identified through experimentation. We plan to work on those optimizations and include performance model--guided scheduling in the future.




==> deleted.tex <==
\begin{figure}[!h]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.45\textwidth,scale=1.0,keepaspectratio]{figures/experiments/google-images/single.png}
  \vspace{-.2in}
  \caption{One tile on one CPU or GPU.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr-single}
\end{figure}

\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}
 \subfloat[4 GPU.\label{subfig-1:page}]{
  \includegraphics[width=0.48\textwidth,scale=1.0,keepaspectratio]{figures/experiments/google-images/Cuda-4-V100-GPUs.png}
  }
   \subfloat[4 CPUs and 1 GPUs.\label{subfig-1:cache}]{
  \includegraphics[width=0.48\textwidth,scale=1.0,keepaspectratio]{figures/experiments/google-images/Cuda-and-OpenMP-4-V100-GPUs-and-1-CPU.png}
  }
   \vspace{-.05in}
   \caption{Scaling and parallelism.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:stream}
 %\vspace{-1.6em}
\end{figure*}
\subsection{Strong Scaling for Large Problems and Graphs
} 


\begin{figure}[!h]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.45\textwidth,scale=1.0,keepaspectratio]{figures/experiments/equinox-scal.png}
  %\vspace{-.2in}
  \caption{Strong scaling in NVIDIA DGX.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr-dgx-scal}
\end{figure}

\begin{figure}[!h]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.45\textwidth,scale=1.0,keepaspectratio]{figures/experiments/mi100-scal.png}
  \vspace{-.05in}
  \caption{Strong scaling in Cades machine with four NVIDIA A100 and four AMD MI100 GPUs.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr-cades-scal}
\end{figure}

\begin{figure}[!h]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.45\textwidth,scale=1.0,keepaspectratio]{figures/experiments/crusher-scal.png}
  \vspace{-.05in}
  \caption{Strong scaling in Frontier node with eight AMD MI150 GPUs.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr-crusher-scal}
\end{figure}

==> one_row_graphs.tex <==

\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}
 \subfloat[Impact of cache line size and page size.\label{subfig-1:page}]{
  \includegraphics[width=0.33\textwidth,scale=1.0,keepaspectratio]{figures/gpu_p100.png}
  }
   \hspace{-1em}
   \subfloat[Impact of array initialization.\label{subfig-1:cache}]{
  \includegraphics[width=0.32\textwidth,scale=1.0,keepaspectratio]{figures/gpu_all.png}
  }
  \hspace{-1em}
  \subfloat[Impact of prefetching on read traffic.\label{subfig-1:prefetch}]{
  \includegraphics[width=0.33\textwidth,scale=1.0,keepaspectratio]{figures/tailored_comparison.png}

  }
   \vspace{-.05in}
   \caption{LLC-DRAM traffic for different read and write scenarios in Intel processors. LLC-DRAM traffic is shown at Y-axis.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:stream}
 \vspace{-1.6em}
\end{figure*}

==> understanding.tex <==
\section{Understanding NVIDIA and AMD GPUs}
\label{label:understanding}
This section explores the similarities and dissimilarities of LLC-memory traffic between Intel CPUs and NVIDIA and AMD GPUs. LLC-memory traffic is measured on the GPUs using the methodologies presented in~\cref{label:methodologies}. The memory traffic is then compared with the memory traffic from the Intel CPUs, as described in \cref{label:background}. Three NVIDIA GPUs are investigated, followed by an exploration of AMD GPUs. All graphs presented in this section show the stride along the x-axis, and the read/write traffic in MB along the y-axis. Through the course of this investigation, some key observations and hypotheses are formulated.

\subsection{LLC-memory traffic of NVIDIA GPUs}
Three NVIDIA GPUs are investigated: Pascal~(P100), Volta~(V100), and Ampere~(A100). 

\begin{figure} [!t]
    \centering
    %\vspace{-0.1in}
    \includegraphics[width=0.4\textwidth,scale=0.7,keepaspectratio]{figures/gpu_p100.png}
    \vspace{-0.05in}
    \caption{Read and write traffic for the P100 GPU. The P100 traffic follows a trend similar to the Skylake CPUs when the write data structure is initialized, and the Intel compiler is used.}
    \label{fig:P100_cpu}
   \vspace{-0.15in}
\end{figure}

\subsubsection{Similarities between P100 GPU and Skylake CPU}
LLC-memory traffic for strided \textit{vecMul} on the P100 is presented in Figure~\ref{fig:P100_cpu}. The blue lines represent the data for the P100. The P100's traffic trend is very similar to the CPU when the write data structure is initialized and compiled using the Intel compiler. Notably, \textit{vecMul} for the GPU does not have the write array initialized. Even though the write array is uninitialized, the P100 shows a trend similar to the CPU with allocating store. The CPU traffic is presented using green lines (the same data from Figure~\ref{fig:back-intel}). In this case, the primary difference is observed for the strides of 8 and 16. This difference is caused by the cache line sizes in the NVIDIA GPU (32 bytes) vs. the Intel CPU (64 bytes). The following observations can be made from the results in Figure~\ref{fig:P100_cpu}.

\textbf{Observation-1} Like the Intel compiler, the \textit{nvcc} compiler implements the streaming-store operation when the stride is 1.

\textbf{Observation-2} The NVIDIA GPU performs the allocating store even when the data structure is not initialized.

\textbf{Observation-3} The NVIDIA GPU's write traffic is the same as the write traffic for the initialized case of the Skylake CPU.

\begin{figure} [!h]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=0.4\textwidth,scale=0.7,keepaspectratio]{figures/gpu_all.png}
    \vspace{-0.05in}
    \caption{Read and write traffic for all NVIDIA GPUs.}
    \label{fig:all_nvidia_gpu}
   \vspace{-0.1in}
\end{figure}

\subsubsection{Similarities between P100, V100, and A100}
Figure~\ref{fig:all_nvidia_gpu} depicts memory traffic from all NVIDIA GPUs studied here. As one can see, the write traffic for all GPUs is the same. Moreover, all GPUs implement streaming store and allocating store. Therefore, Observations 1, 2, and 3 are also applicable for V100 and A100. For both read and write traffic, V100 and A100 show little to no difference. The main difference between P100 and later GPUs is observed for the read traffic when the stride size is larger than the cache line size (stride of 8). On average, the read traffic for V100 and A100 is $1.6\times$ higher than for P100. When the stride size is larger than the cache line size, the difference between P100 and A100 (also V100) shows a striking similarity to the prefetching-enabled and disabled cases for Intel CPUs presented in Figure~\ref{fig:back-pref}. This difference suggests that a major change was applied to the prefetchers of the Volta architecture and onward. Therefore, the following observation and hypothesis can be made.

\textbf{Observation-4} When the stride size is larger than the cache line on V100 and A100 GPUs, the read traffic shows a similar pattern to the prefetching-enabled Skylake CPU. Traffic is about $1.6\times$ higher than on the P100 and on the prefetching-disabled Skylake CPU.

\textbf{Hypothesis-1} From the Volta GPU architecture onward, NVIDIA GPUs implement an Intel CPU--like prefetching mechanism.

\begin{figure} [!h]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=0.4\textwidth,scale=0.7,keepaspectratio]{figures/tailored_comparison.png}
    \vspace{-0.05in}
    \caption{Tailored comparison between NVIDIA GPUs and Intel CPU.}
    \label{fig:tailored_gpu}
   \vspace{-0.1in}
\end{figure}


\subsubsection{A tailored graph to realize the similarities}
A hypothetical scenario is considered in which the cache line size of the Skylake CPU is 32 bytes instead of 64 bytes to demonstrate the similarities between the Intel CPU and the NVIDIA GPUs. Even though the consideration is hypothetical, the data presented in Figure~\ref{fig:tailored_gpu} are actual data. To prepare Figure~\ref{fig:tailored_gpu}, the read and write traffic for stride 16 is removed only for the CPU and shifted to the left for all strides greater than 16. This conversion shows the CPU data for a 32-byte cache line because one read or write would fetch/store 32 bytes instead of 64 bytes. The highest stride shown in Figure~\ref{fig:tailored_gpu} is 4,096 instead of 8,192. After this conversion, the write traffic for all GPUs and the CPU shows similar data and trends. The similarity is observed between the read traffic for the P100 and the CPU with prefetching disabled (see the overlapped blue and black lines in Figure~\ref{fig:tailored_gpu} for the read traffic). 

All GPUs and the CPU in Figure~\ref{fig:tailored_gpu} show similar data for the read traffic until a stride of 8. The A100, V100, and the prefetching-enabled CPU show the same trend after a stride size of 8 (denoted by green and red lines in Figure~\ref{fig:tailored_gpu}). However, there is no overlap between the green and red lines, and the CPU reports higher read traffic than the A100 GPU until stride 64, and then the opposite is observed. The CPU keeps prefetching until stride 80, which is not shown in the figure and is determined experimentally. In contrast, the GPU keeps prefetching even for higher strides where there should not be any benefit for such action because the memory accesses are more than four cache lines apart. In summary, it can be said that there are more similarities than dissimilarities. Therefore, the following hypothesis can be formulated.

\textbf{Hypothesis-2} A model prepared to predict LLC-memory traffic for sequential streaming and strided access patterns for an Intel Skylake CPU with a cache line size of 32 bytes can be customized to predict LLC-memory traffic for NVIDIA GPUs.



\subsection{LLC-memory traffic of AMD GPUs}
Compared with the NVIDIA GPUs, the AMD GPUs considered in this study are relatively new. The MI50 and MI60 Instinct GPUs have the same GCN 5.1 architecture, whereas MI100 adopts a CDNA 1.0 architecture. Because these GPUs were released within two years, similarity is expected. 

\begin{figure} [!h]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=0.4\textwidth,scale=0.7,keepaspectratio]{figures/mi50_cpu.png}
    \vspace{-0.05in}
    \caption{Read and write traffic for the MI50 GPU compared with the Intel Skylake CPU.}
    \label{fig:mi50_cpu}
   \vspace{-0.1in}
\end{figure}




\subsubsection{Similarities between MI50 GPU and Skylake CPU}
The LLC-memory traffic for MI50 is shown in Figure~\ref{fig:mi50_cpu}. The read and write traffic for stride 1 is very close to the theoretical lower bound. The read traffic in Figure~\ref{fig:mi50_cpu} for MI50 follows the same trend as the Skylake CPU when the data structure is not initialized (shown initially in Figure~\ref{fig:back-init-non-init}). The \textit{vecMul} function for the GPU does not have the write array initialized. So, unlike NVIDIA GPUs, the MI50 does not implement allocating store, which is more appropriate for this function because there is no value in the write array, and bringing the cache line from memory is unnecessary. 

\textbf{Observation-5} AMD GPUs do not implement allocating store for an uninitialized write array.

Even though the read traffic shows similarity with the non-initialized case, the write traffic in Figure~\ref{fig:mi50_cpu} shows the same trend as the write traffic for the initialized case. Hence, it proves that page zeroing, like on the CPU, is not occurring even though the write array is not initialized. 

The most interesting observation in Figure~\ref{fig:mi50_cpu} is that a drop in read traffic occurs when the stride is 16, but a drop in write traffic occurs when the stride is 8. This difference suggests that the cache line length is 64 bytes for the read transactions and 32 bytes for the write transactions. Such a scenario is not observed in Intel CPUs or NVIDIA GPUs.  To confirm the cache line length, the \textit{rocminfo} command is used in all AMD GPUs, in which the cache line length is 64 bytes. The write traffic dropping at a stride of 8 instead of 16, even though the cache line length is 64 bytes, must be investigated. 

To investigate this anomaly, the metric used to measure the write traffic is explored. The metric's formula is \textit{WRITE\_SIZE = (TCC\_MC\_WRREQ\_sum*32) / 1024} (this formula is found in the metrics.xml file inside the ROCm software stack's rocprofiler directory). The metric is described as, \quotes{The total kilobytes fetched from the video memory. This is measured with all extra fetches and any cache or memory effects taken into account.} For further investigation, the \textit{TCC\_MC\_WRREQ\_sum} metric is explored, where the formula is \textit{sum(TCC\_MC\_WRREQ,16)}. The metric is described as, \quotes{Number of 32-byte transactions going over the \textit{TC\_MC\_wrreq} interface. Sum over TCC instances.} This description confirms that AMD GPUs perform 32-byte transactions for write traffic, and the write traffic in AMD GPUs follows the same trend as the NVIDIA GPUs. 

\textbf{Observation-6} AMD GPUs show 64-byte LLC-memory transactions for read traffic and 32-byte transactions for write traffic.

\begin{figure} [!h]
    \centering
    \vspace{-0.1in}
    \includegraphics[width=0.4\textwidth,scale=0.7,keepaspectratio]{figures/all_amd_gpu.png}
    \vspace{-0.05in}
    \caption{Read and write traffic for all AMD GPUs.}
    \label{fig:all_amd_gpu}
   \vspace{-0.1in}
\end{figure}


\subsubsection{Similarities between MI50, MI60, and MI100}
The LLC-memory traffic for MI50, MI60, and MI100 is shown in Figure~\ref{fig:all_amd_gpu}. All AMD GPUs show similar trends and data. Therefore, Observations 4 and 5 apply to all AMD GPUs (transitive property), and the following hypothesis can be~made.

\textbf{Hypothesis-3} Because of the many similarities, a model prepared to predict LLC-memory traffic for sequential streaming and strided access patterns for an Intel Skylake CPU can be customized to predict LLC-memory traffic for AMD~Instinct~GPUs.




\subsection{Comparison of the profiling tools}
\label{label:profiling_tools}
This study found that NVIDIA's \textit{ncu} tool provides more hardware counters and metrics for GPU execution than AMD's \textit{rocprof}. However, the detailed formula behind a metric can be found in \textit{rocprof}, which is helpful for further investigation. Moreover, \textit{rocprof} provides the facility to write custom-derived metrics. From an accuracy standpoint, both \textit{ncu} and \textit{rocprof} provide reasonably accurate traffic counts that are close to the theoretical traffic count for lower strides. Unfortunately, this is not the case for CPUs. Our previous study observed some extra traffic while measuring CPUs. One common problem found for all cases is that when the number of accesses is low (i.e., higher strides), the traffic count is not accurate when compared with the theoretical traffic. Based on this study, it is possible that the inaccuracies in higher strides come from having low memory access and an application with a shorter lifespan. A shorter application lifespan makes pinpointing the memory traffic of a function difficult for the profiler. While modeling and comparing accuracy, this factor must be taken into consideration.


\subsection{Discussion about the hypotheses}
Three hypotheses are formulated in this study. To prove Hypothesis-1, one would need to study the details of the changes in NVIDIA's prefetching algorithm from Pascal to Volta. However, Hypotheses 2 and 3 can be verified by preparing a prediction model. 

%similarly adopted in our previous tudy~\cite{monil:2020:Understanding}.


==> unused_text.tex <==



\begin{figure*}[htp]
\centering 
\begin{minipage}{1\linewidth}
\small
%\begin{listing}
\begin{minted}[linenos=true, breaklines, breakafter=d, fontsize=\scriptsize, frame=single, encoding=utf8]{c}
// Creation of the IRIS graph
iris_graph graph; iris_graph_create(&graph);
iris_task getrf_tasks[TILE_NUM*TILE_NUM], trsm_tasks[TILE_NUM*TILE_NUM], gemm_tasks[TILE_NUM*TILE_NUM*TILE_NUM];
// Tiled LU factorization
for ( int step = 0; step < TILE_NUM; step++ ) {
  // GETRF tasks
  iris_task_create( &getrf_tasks[(step*TILE_NUM)+step] );
  // Dependencies for getrf tasks
  if ( step > 0 ){
    iris_task getrf_depend_tasks[] = { gemm_tasks[((step-1)*TILE_NUM*TILE_NUM)+((step*TILE_NUM)+step)] };
    iris_task_depend( getrf_tasks[(step*TILE_NUM)+step], 1, getrf_depend_tasks );
  }
  // Encapsulate GETRF tasks into the graph 
  laris_getrf_graph( graph, getrf_tasks[(step*TILE_NUM)+step], step, step, step,
        TILE_SIZE, TILE_SIZE, IRIS_Ctile[step*TILE_NUM+step], A_tile[step][step], TILE_SIZE );
  for ( int tile_jj = 1 + step; tile_jj < TILE_NUM; tile_jj++ ) {
    // trsm tasks
    iris_task_create( &trsm_tasks[(step*TILE_NUM)+tile_jj] );
    // Dependencies for trsm tasks
    if ( step == 0 ) {
      iris_task trsm_depend_tasks[] = { getrf_tasks[ ( step * TILE_NUM ) + step ] };
      iris_task_depend( trsm_tasks[(step*TILE_NUM)+tile_jj], 1, trsm_depend_tasks );
    } else {
        iris_task trsm_depend_tasks[] = { getrf_tasks[(step*TILE_NUM)+step], 
                  gemm_tasks[((step-1)*TILE_NUM*TILE_NUM)+(step*TILE_NUM)+tile_jj]};
        iris_task_depend( trsm_tasks[(step*TILE_NUM)+tile_jj], 2, trsm_depend_tasks );
    }
    // Encapsulate trsm tasks into the graph 
    laris_trsm_top_graph( graph, trsm_tasks[(step*TILE_NUM)+tile_jj], step, step, tile_jj,
          TILE_SIZE, TILE_SIZE, IRIS_Ctile[step*TILE_NUM+step],    A_tile[step][step],    TILE_SIZE,
          IRIS_Ctile[step*TILE_NUM+tile_jj], A_tile[step][tile_jj], TILE_SIZE );
  }
  for ( int tile_ii = 1 + step; tile_ii < TILE_NUM; tile_ii++ ) {
    // trsm tasks
    iris_task_create( &trsm_tasks[(tile_ii*TILE_NUM)+step] );
    // Dependencies for trsm tasks
    if ( step == 0 ) {
      iris_task trsm_depend_tasks[] = { getrf_tasks[ ( step * TILE_NUM ) + step ]};
      iris_task_depend( trsm_tasks[ ( tile_ii * TILE_NUM ) + step ], 1, trsm_depend_tasks );
    } else {
      iris_task trsm_depend_tasks[] = { getrf_tasks[(step*TILE_NUM)+step], 
                gemm_tasks[((step-1)*TILE_NUM*TILE_NUM)+(tile_ii*TILE_NUM)+step] };
      iris_task_depend( trsm_tasks[ ( tile_ii * TILE_NUM ) + step ], 2, trsm_depend_tasks );
    }
    // Encapsulate trsm tasks into the graph
    laris_trsm_left_graph( graph, trsm_tasks[(tile_ii*TILE_NUM)+step], step, tile_ii, step,
          TILE_SIZE, TILE_SIZE, IRIS_Ctile[step * TILE_NUM + step], A_tile[step][step],
          TILE_SIZE, IRIS_Ctile[tile_ii * TILE_NUM + step], A_tile[tile_ii][step], TILE_SIZE );
    }
    for ( int tile_i = step + 1; tile_i < TILE_NUM; tile_i++ ) {
      for ( int tile_j = step + 1; tile_j < TILE_NUM; tile_j++ ) {
        // gemm tasks
        iris_task_create( &gemm_tasks[(step*TILE_NUM*TILE_NUM)+((tile_i*TILE_NUM)+tile_j)] );
        // Dependencies for gemm tasks
        if ( step == 0 ) {
          iris_task gemm_depend_tasks[] = { trsm_tasks[(tile_i*TILE_NUM)+step], trsm_tasks[(step*TILE_NUM)+tile_j] };
          iris_task_depend( gemm_tasks[(step*TILE_NUM*TILE_NUM)+((tile_i*TILE_NUM)+tile_j)], 2, gemm_depend_tasks );
        } 
        else {
           iris_task gemm_depend_tasks[] = {  trsm_tasks[(tile_i*TILE_NUM)+step], trsm_tasks[(step*TILE_NUM)+tile_j],
                     gemm_tasks[((step-1)*TILE_NUM*TILE_NUM)+((tile_i*TILE_NUM)+tile_j)] };
           iris_task_depend( gemm_tasks[(step*TILE_NUM*TILE_NUM)+((tile_i*TILE_NUM)+tile_j)], 3, gemm_depend_tasks );
        }
        // Encapsulate gemm tasks into the graph 
        laris_gemm_graph( graph, gemm_tasks[(step*TILE_NUM*TILE_NUM)+((tile_i*TILE_NUM)+tile_j)],
              step, tile_i, tile_j, TILE_SIZE, TILE_SIZE, TILE_SIZE, -1.0, IRIS_Ctile[tile_i*TILE_NUM+step],
              A_tile[tile_i][step], TILE_SIZE, IRIS_Ctile[step*TILE_NUM+tile_j],  A_tile[step][ tile_j], TILE_SIZE, 1.0, 
              IRIS_Ctile[tile_i*TILE_NUM+tile_j], A_tile[tile_i][tile_j], TILE_SIZE );
}}}
iris_graph_submit(graph, iris_default, 1);
\end{minted}
\end{minipage}
\caption{Tiled LU factorization code of LaRIS.}
    \label{lst:getrf_code}
\end{figure*}


\begin{figure}[htp]
\centering 
\begin{minipage}{0.9\linewidth}
%\begin{listing}
\begin{minted}[linenos=true, breaklines, breakafter=d, fontsize=\scriptsize, frame=single, encoding=utf8]{c}
int laris_gemm_graph( 
    iris_graph graph, 
    iris_task T, 
    int step, int tile_i, int tile_j, 
    int M, int N, int K, 
    TYPE ALPHA, iris_mem d_A, TYPE *h_A, int LDA, 
    iris_mem d_B, TYPE *h_B, int LDB, 
    TYPE BETA, iris_mem d_C, TYPE *h_C, int LDC )
{
  // Memory communication -> input
  iris_task_h2d(T, d_A, 0, M*K*sizeof(TYPE), h_A);
  iris_task_h2d(T, d_B, 0, K*N*sizeof(TYPE), h_B);
  iris_task_h2d(T, d_C, 0, M*N*sizeof(TYPE), h_C);
  // IRIS-BLAS call
  iris_core_nodt_gemm( T, IRIS_BLAS_COL_MAJOR, 
        IRIS_BLAS_NO_TRANS, IRIS_BLAS_NO_TRANS, 
        M, N, K, ALPHA, d_A, LDA, 
        d_B, LDB,BETA, d_C, LDC); 
  // Memory communication -> output
  iris_task_d2h(T, d_C, 0, M*N*sizeof(TYPE), h_C);
  iris_graph_task( graph, T, iris_any, NULL );
  return 0;
}
\end{minted}
\end{minipage}
\caption{gemm code of LaRIS.}
    \label{lst:gemm_code}
\end{figure}




\begin{figure}[!th]
 \centering
  %\vspace*{-2.em}

   \subfloat[Strong scaling in NVIDIA DGX.\label{subfig-2:cades}]{
  \includegraphics[width=.4\textwidth,scale=1.0,keepaspectratio]{figures/experiments/equinox-scal.png}
  }

  \subfloat[Frontier node with eight AMD MI150 GPUs.\label{subfig-2:dgx}]{
  \includegraphics[width=.4\textwidth, scale=1.0,keepaspectratio]{figures/experiments/crusher-scal.png}
  }
  
   \subfloat[Cades node with four NVIDIA A100 and four AMD MI100 GPUs.\label{subfig-2:crusher}]{
  \includegraphics[width=.4\textwidth,scale=1.0,keepaspectratio]{figures/experiments/mi100-scal.png}
  }
  
   \vspace{-.05in}
   \caption{Strong scaling in different machine.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr:strong-scaling}
 %\vspace{-1.6em}
\end{figure}

\begin{figure}[!h]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.45\textwidth,scale=1.0,keepaspectratio]{figures/experiments/task_scalability.png}
  \vspace{-.05in}
  \caption{Trade-off between overhead and parallelism in an NVIDIA DGX node with one Intel CPU and four NVIDIA GPUs}
 \label{fig:expr-crusher-scal}
\end{figure}


\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/Equinox-32k-32.png}
  \vspace{-.2in}
  \caption{Exploiting parallelism in an NVIDIA DGX. Red=GETRF, Orange=TRSM and Blue=GEMM.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:trace-equinox}

\end{figure*}


\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/mi100-16k-32.png}
  \vspace{-.2in}
  \caption{Exploiting parallelism in an Multi-vendor GPUs along with a CPU. Red=GETRF, Orange=TRSM and Blue=GEMM.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:trace-mi100}

\end{figure*}


\begin{figure*}[!th]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.75\textwidth,scale=1.0,keepaspectratio]{figures/crusher-16k-32.png}
  \vspace{-.2in}
  \caption{Frontier trace. Red=GETRF, Orange=TRSM and Blue=GEMM.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:trace-mi100}

\end{figure*}

\begin{figure}[!h]
 \centering
  %\vspace*{-2.em}
  \includegraphics[width=.45\textwidth,scale=1.0,keepaspectratio]{figures/experiments/google-images/Scalability-Frontier.png}
  \vspace{-.2in}
  \caption{Strong scaling Frontier node.
   %Y axis = LLC-DRAM traffic measurement by the dynamic analysis tool and X axis = the stride size.
   }
 \label{fig:expr-single}
\end{figure}

\begin{table*}[!b]
%\vspace{-0.1 in}
\caption[NVIDIA GPUs studied in Chapter VI.]{NVIDIA GPUs.}
%\vspace{-0.1 in}
%\small
\centering
%\setlength{\tabcolsep}{0.4em}
\begin{center}
%\begin{tabular}{| P{1.2cm} | p{6.8cm} |}

\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Item} &\multicolumn{4}{|c|}{\textbf{NVIDIA Tesla GPUs }}  \\
\cline{2-5} 
 \textbf{description} & \textbf{\textit{Pascal: P100}} & \textbf{\textit{Volta: V100}} & \textbf{\textit{Ampere: A100}} & \textbf{\textit{Hopper: H100}}\\
\hline
%    \textbf{Kernel name} & \textbf{Operational Intensity} & \textbf{Total Flop} & \textbf{CPU Flop/s} & \textbf{}\\ \hline 
Release year & 2016 & 2017 &  2020 & 2022   \\ \hline
Architecture & Pascal & Volta &  Ampere & Hopper \\ \hline
Number of SMs/CUs & 56 & 80 & 108  & 114   \\  \hline
Number of cores & 3,584 & 5,120  & 6,912 & 14592\\  \hline
%Peak performance FP16 (half) & 19.05 TFLOPS &    28.26 TFLOPS & 77.97 TFLOPS & 26.82 TFLOPS & 29.49 TFLOPS  & 184.6 TFLOPS \\  \hline
Peak performance FP32 & 13.41 TFLOPS &   14.13 TFLOPS & 19.49 TFLOPS & 48 TFLOPS \\  \hline
Peak performance FP64 & 6.705 TFLOPS &   7.066 TFLOPS & 9.746 TFLOPS & 24 TFLOPS\\  \hline
Tensor/Matrix cores & No & Yes (640) & Yes (432)  & Yes (456)   \\  \hline
Device memory size & 16 GB HBM2 & 16 GB HBM2 & 40 GB HBM2e & 80 GB HBM3 \\  \hline
Memory bus & 4,096 bit & 4,096 bit & 5,120 bit & 5,120 bit \\  \hline
Bandwidth & 732.2 GB/s
 & 900 GB/s  & 1,555 GB/s  & 1920 GB/s  \\  \hline
L1 cache per SM/CU & 24 KB & 128 KB  & 192 KB & 256 KB  \\  \hline
L2 cache size & 4 MB & 6 MB &  40 MB & 50 MB\\  \hline
Cache line size & 32 bytes & 32 bytes &  32 bytes & 32 bytes   \\  \hline
Warp/Wavefront size & 32 threads & 32 threads &    32 threads & 32 threads   \\  \hline

Compiler & nvcc & nvcc & nvcc & nvcc \\  \hline

Profiler & nvprof & nvprof & Nsight compute & Nsight compute  \\  \hline
Software stack & CUDA-11.0 & CUDA-11.2 & CUDA-11.2 & CUDA-11.x\\  \hline

Machine name & Oswald01 & Leconte & Illyad & none \\  \hline

Facility & ExCL & ExCL & OACISS & none \\  \hline

\end{tabular}

\label{table:gpus}
\end{center}
%\vspace{-0.05in}
\end{table*}



\begin{table*}[!b]
%\vspace{-0.1 in}
\caption[AMD GPUs studied in Chapter VI.]{AMD GPUs.}
%\vspace{-0.1 in}
%\small
\centering
%\setlength{\tabcolsep}{0.4em}
\begin{center}
%\begin{tabular}{| P{1.2cm} | p{6.8cm} |}

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Item} & \multicolumn{4}{|c|}{\textbf{AMD Radeon Instinct GPUs }} \\
\cline{2-5} 
 \textbf{description} & \textbf{\textit{MI50}} & \textbf{\textit{MI60}} & \textbf{\textit{MI100}} & \textbf{\textit{MI250}}\\
\hline
%    \textbf{Kernel name} & \textbf{Operational Intensity} & \textbf{Total Flop} & \textbf{CPU Flop/s} & \textbf{}\\ \hline 
Release year  & 2018 & 2018 & 2020 & 2021 \\ \hline
Architecture  & GCN 5.1 & GCN 5.1 & CDNA 1.0 & CDNA 2.0 \\ \hline
Number of SMs/CUs   &  60 & 64 &  120  & 208 \\  \hline
Number of cores     & 3,840 & 4,096  & 7,680 & 13312 \\  \hline
%Peak performance FP16 (half) & 19.05 TFLOPS &    28.26 TFLOPS & 77.97 TFLOPS & 26.82 TFLOPS & 29.49 TFLOPS  & 184.6 TFLOPS \\  \hline
Peak performance FP32 & 13.41 TFLOPS  & 14.75 TFLOPS & 23.07 TFLOPS & 45 TFLOPS  \\  \hline
Peak performance FP64 & 6.705 TFLOPS & 7.373 TFLOPS  & 11.54 TFLOPS & 45 TFLOPS\\  \hline
Tensor/Matrix cores & No & No & Yes (each CU) & Yes (880) \\  \hline
Device memory size   & 16 GB HBM2 & 32 GB HBM2 & 32 GB HBM2 & 128 GB HBM2e \\  \hline
Memory bus  & 4,096 bit & 4,096 bit & 4,096 bit & 8192 bit \\  \hline
Bandwidth  & 1,024 GB/s  & 1,024 GB/s & 1,229 GB/s & 3222 GB/s\\  \hline
L1 cache per SM/CU   & 16 KB & 16 KB & 16 KB & 16 KB \\  \hline
L2 cache size  &  4 MB & 4 MB & 8 MB & 16 MB \\  \hline
Cache line size  & 64 bytes & 64 bytes & 64 bytes & 64 bytes\\  \hline
Warp/Wavefront size & 64 threads & 64 threads & 64 threads & 64 threads  \\  \hline

Compiler & hipcc & hipcc  & hipcc & amdclang \\  \hline

Profiler & rocprof & rocprof  & rocprof & rocprof \\  \hline
Software stack & ROCm-3.9.0 & ROCm-4.3.0  & ROCm-4.3.0 & ROCm-5.x \\  \hline

Machine name & Gilgamesh & Explorer & Cousteau & Crusher \\  \hline

Facility & OACISS & ExCL & ExCL & OLCF \\  \hline

\end{tabular}

\label{table:gpus_amd}
\end{center}
%\vspace{-0.05in}
\end{table*}




\begin{table*}[!b]
%\vspace{-0.1 in}
\caption[AMD GPUs studied in Chapter VI.]{Intel GPUs.}
%\vspace{-0.1 in}
%\small
\centering
%\setlength{\tabcolsep}{0.4em}
\begin{center}
%\begin{tabular}{| P{1.2cm} | p{6.8cm} |}

\begin{tabular}{|c|c|}
\hline
\textbf{Item} & \multicolumn{1}{|c|}{\textbf{Intel}} \\
%\cline{} 
 \textbf{description} & \textbf{\textit{Xe-HPC}} \\
\hline
%    \textbf{Kernel name} & \textbf{Operational Intensity} & \textbf{Total Flop} & \textbf{CPU Flop/s} & \textbf{}\\ \hline 
Release year  & Not yet  \\ \hline
Architecture  & Xe \\ \hline
Number of SMs/CUs/Xe   &  128  \\  \hline
Number of cores     &  16 per Xe\\  \hline
%Peak performance FP16 (half) & 19.05 TFLOPS &    28.26 TFLOPS & 77.97 TFLOPS & 26.82 TFLOPS & 29.49 TFLOPS  & 184.6 TFLOPS \\  \hline
Peak performance FP32 & NA    \\  \hline
Peak performance FP64 & NA \\  \hline
Tensor/Matrix cores & 16 matrix engine per Xe core  \\  \hline
Device memory size   & 16 GB HBM2e  \\  \hline
Memory bus  & 4,096 bit  \\  \hline
Bandwidth  & NA \\  \hline
L1 cache per SM/CU   & 512 KB  \\  \hline
L2 cache size  &  144 MB  \\  \hline
Cache line size  & 64 bytes \\  \hline
Warp/Wavefront size &  NA \\  \hline
Compiler &  NA \\  \hline
Profiler & Vtune  \\  \hline
Software stack & OpenAPI \\  \hline

Machine name & none  \\  \hline

Facility & none  \\  \hline

\end{tabular}

\label{table:gpus_intel}
\end{center}
%\vspace{-0.05in}
\end{table*}
